A Unified Model for Reverse Dictionary and Definition Modelling

We build a dual-way neural dictionary to retrieve words given definitions, and produce definitions for queried words. The model learns the two tasks simultaneously and handles unknown words via embeddings. It casts a word or a definition to the same representation space through a shared layer, then generates the other form in a multi-task fashion. Our method achieves promising automatic scores on previous benchmarks without extra resources. Human annotators prefer the model's outputs in both reference-less and reference-based evaluation, indicating its practicality. Analysis suggests that multiple objectives benefit learning.

==> train_plots.tex <==
\begin{figure}[h]
\centering
\resizebox{0.24\textwidth}{!}{%
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group name=revdic,
        group size=1 by 2
    },
    width=6cm,
    xmin=0, xmax=20,
    xlabel=(a) reverse dictionary
]

\nextgroupplot[ymin=0.0285,ymax=0.0315,
               axis y line=left,
               axis x line=bottom,
               height=6cm]
\addplot[
    color=cyan,
    mark=o,
    ]
    coordinates {
    (0,0.0687)(1,0.0328)(2,0.0304)(3,0.0301)(5,0.0300)(8,0.0299)(9,0.0298)
    };
    % \addlegendentry{1-task};
\addplot[
    color=blue,
    mark=triangle,
    ]
    coordinates {
    (0,0.0303)(4,0.0299)(5,0.0296)(6,0.0295)(7,0.0294)(8,0.0291)(10,0.0289)(11,0.0289)(13,0.0288)(15,0.0288)(17,0.0287)(18,0.0286)%(34,0.0286)
    };
    % \addlegendentry{3-task};
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (0,0.0303)(4,0.0300)(5,0.0298)(6,0.0297)(7,0.0295)(8,0.0293)(9,0.0293)(10,0.0291)(12,0.0289)(17,0.0289)(18,0.0287)(19,0.0286)
    };
    % \addlegendentry{5-task};

\end{groupplot}
\end{tikzpicture}
}%
\resizebox{0.24\textwidth}{!}{%
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group name=defmod,
        group size=1 by 2
    },
    width=6cm,
    % xmin=0, xmax=5,
    xlabel=(b) definition modelling,
    legend cell align={left}
]

\nextgroupplot[ymin=3.8,ymax=5.5,
            %   ytick={4,5,6},
               axis y line=left,
               axis x line=bottom,
               height=5.5cm]
\addplot[
    color=cyan,
    mark=o,
    ]
    coordinates {
    (0,5.2527)(1,4.8284)(2,4.4563)(3,4.1856)(4,4.0236)(5,3.9176)
    };
    \addlegendentry{Transformer};
\addplot[
    color=blue,
    mark=triangle,
    ]
    coordinates {
    (0,5.0704)(1,4.5802)(2,4.2917)(3,4.1786)(4,4.1468)
    };
    \addlegendentry{ours};
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (0,5.4544)(1,4.8312)(2,4.3971)(3,4.0946)(4,3.9820)(5,3.9284)
    };
    \addlegendentry{ours+embed};

\end{groupplot}

\end{tikzpicture}
}%
\caption{Training losses (y-axis) against epochs (x-axis).}
\vspace{-1ex}
\label{fig:train_losses}
\end{figure}
